A Causal Perspective on Meaningful and Robust Algorithmic Recourse

Algorithmic recourse explanations inform stakeholders on how to act to revert unfavorable predictions. However, in general ML models do not predict well in interventional distributions. Thus, an action that changes the prediction in the desired way may not lead to an improvement of the underlying target. Such recourse is neither meaningful nor robust to model refits. Extending the work of Karimi et al. (2021), we propose meaningful algorithmic recourse (MAR) that only recommends actions that improve both prediction and target. We justify this selection constraint by highlighting the differences between model audit and meaningful, actionable recourse explanations. Additionally, we introduce a relaxation of MAR called effective algorithmic recourse (EAR), which, under certain assumptions, yields meaningful recourse by only allowing interventions on causes of the target.

==> latex-math/basic-math.tex <==
% math spaces
\ifdefined\N                                                                % N, naturals
\renewcommand{\N}{\mathds{N}}                                                % N defined by "siunitx" (which we use), for "NEWTON"
\else
  \newcommand{\N}{\mathds{N}}
\fi
\newcommand{\Z}{\mathds{Z}}                                                 % Z, integers
\newcommand{\Q}{\mathds{Q}}                                                 % Q, rationals
\newcommand{\R}{\mathds{R}}                                                 % R, reals
\ifdefined\C
  \renewcommand{\C}{\mathds{C}}                                             % C, complex
\else
  \newcommand{\C}{\mathds{C}}
\fi
\newcommand{\HS}{H}                                               % H, hilbertspace
\newcommand{\continuous}{\mathcal{C}}                                       % C, space of continuous functions
\newcommand{\M}{\mathcal{M}} 												% machine numbers
\newcommand{\epsm}{\epsilon_m} 												% maximum error

% counting / finite sets
\newcommand{\setn}{\{1, \ldots, n\}} 											% {1, ..., n}
\newcommand{\setp}{\{1, \ldots, p\}}											% {1, ..., p}
\newcommand{\setg}{\{1, \ldots, g\}}											% {1, ..., g}
\newcommand{\setzo}{\{0, 1\}} 		        			    				% {0, 1}
\newcommand{\setmp}{\{-1, +1\}}     				    					% {-1, 1}


% basic math stuff
\newcommand{\xt}{\tilde x}													% x tilde
\def\argmax{\mathop{\sf arg\,max}}                                          % argmax
\def\argmin{\mathop{\sf arg\,min}}                                          % argmin
\newcommand{\sign}{\operatorname{sign}}                                     % sign, signum
\newcommand{\I}{\mathbb{I}}                                                 % I, indicator
\newcommand{\order}{\mathcal{O}}                                            % O, order
\newcommand{\fp}[2]{\frac{\partial #1}{\partial #2}}                        % partial derivative
\newcommand{\pd}[2]{\frac{\partial{#1}}{\partial #2}}						% partial derivative

% sums and products
\newcommand{\sumin}{\sum\limits_{i=1}^n}											% summation from i=1 to n
\newcommand{\sumjp}{\sum\limits_{j=1}^p}											% summation from j=1 to p
\newcommand{\sumik}{\sum\limits_{i=1}^k}											% summation from i=1 to k
\newcommand{\sumkg}{\sum\limits_{k=1}^g}											% summation from k=1 to g
\newcommand{\sumjg}{\sum\limits_{j=1}^g}											% summation from j=1 to g
\newcommand{\meanin}{\frac{1}{n} \sum\limits_{i=1}^n}			    				% mean from i=1 to n
\newcommand{\meankg}{\frac{1}{g} \sum\limits_{k=1}^g}			    				% mean from k=1 to g
\newcommand{\prodin}{\prod\limits_{i=1}^n}											% product from i=1 to n
\newcommand{\prodkg}{\prod\limits_{k=1}^g}											% product from k=1 to g
\newcommand{\prodjp}{\prod\limits_{j=1}^p}											% product from j=1 to p

% linear algebra
\newcommand{\one}{\boldsymbol{1}}                                           % 1, unitvector
\newcommand{\zero}{\mathbf{0}}													% 0-vector
\newcommand{\id}{\boldsymbol{I}}                                                % I, identity
\newcommand{\diag}{\operatorname{diag}}                                     % diag, diagonal
\newcommand{\trace}{\operatorname{tr}}                                      % tr, trace
\newcommand{\spn}{\operatorname{span}}                                      % span
\newcommand{\scp}[2]{\left\langle #1, #2 \right\rangle}                     % <.,.>, scalarproduct
\newcommand{\mat}[1]{ 														% short pmatrix command
	\begin{pmatrix}
		#1
	\end{pmatrix}
}
\newcommand{\Amat}{\mathbf{A}}													% matrix A
\newcommand{\xv}{\mathbf{x}}													% vector x (bold)
\newcommand{\yv}{\mathbf{y}}													% vector y (bold)
\newcommand{\Deltab}{\mathbf{\Delta}}											% error term for vectors


% basic probability + stats
\renewcommand{\P}{\mathds{P}}                                               % P, probability
\newcommand{\E}{\mathds{E}}                                                 % E, expectation
\newcommand{\var}{\mathsf{Var}}                                             % Var, variance
\newcommand{\cov}{\mathsf{Cov}}                                             % Cov, covariance
\newcommand{\corr}{\mathsf{Corr}}                                           % Corr, correlation
\newcommand{\normal}{\mathcal{N}}                                           % N of the normal distribution
\newcommand{\iid}{\overset{i.i.d}{\sim}}                                    % dist with i.i.d superscript
\newcommand{\distas}[1]{\overset{#1}{\sim}}                                 % ... is distributed as ...


==> latex-math/ml-automl.tex <==


% lambdav
\newcommand{\lambdav}{\bm{\lambda}}											% lambda vector



==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(x)}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(x)}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(x)}                    % ensembled predictor
\newcommand{\fMh}{\hat f^{[M]}(x)}                    % estimated ensembled predictor
\newcommand{\ambifM}{\Delta\left(\fM\right)}          % ambiguity/instability of ensemble


==> latex-math/ml-bayesopt.tex <==
% ml - Bayesian Optimization

\newcommand{\minit}{m_{\text{init}}											% Size of the initial design
\newcommand{\lambdai}{\lambda^{[i]}											% input for black box optimization 
\newcommand{\lambdaopt}{\lambda^{*}}											% Minimum of the black box function Psi
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\left(\lambda^{[1]}, \dots, \lambda^{[\minit]}\right)}  % Vector of different inputs


% \newcommand{\metadata}



\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process 


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{r^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{r^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}

==> latex-math/ml-feature-sel.tex <==
% ml - feature selection

\newcommand{\xjNull}{x_{j_0}}
\newcommand{\xjEins}{x_{j_1}}
\newcommand{\xl}{\mathbf{x}_l}
\newcommand{\pushcode}[1][1]{\hskip\dimexpr#1\algorithmicindent\relax}

==> latex-math/ml-gp.tex <==
% ml - Gaussian Process

\newcommand{\gp}{\mathcal{GP}\left(m(\bm{x}), k\left(\bm{x}, \bm{x}^\prime\right)\right)} 								% Gaussian Process Definition	
\newcommand{\mvec}{\mathbf{m}}												    						% Gaussian process mean vector
\newcommand{\Kmat}{\mathbf{K}}																			% estimated base learner 
\newcommand{\ls}{\ell}                                           % length-scale


==> latex-math/ml-lm.tex <==
\newcommand{\thx}{\thetab^T \xv}												% linear score: theta^T x



==> latex-math/ml-mbo.tex <==
% ml - MBO
\newcommand{\sxh}{\hat{s}(x)} % uncertainty shat(x)
\newcommand{\vxh}{\hat{s}^2(x)}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\kstarx}{\mathbf{k}_*(x)}
\newcommand{\xpi}[1][i]{x^{*(#1)}}
\newcommand{\vhx}{\ensuremath{\sh^2(\xv)}\xspace}          % local estimated variance at point x
\newcommand{\shx}{\ensuremath{\sh(\xv)}\xspace}            % local estimated uncertainty at point x
\newcommand{\sh}{\ensuremath{\hat{s}}\xspace}              % local estimated uncertainty
\newcommand{\px}{\ensuremath{\boldsymbol{x}^*}}
\newcommand{\equote}[1]{``#1''}
\newcommand{\vecx}{\ensuremath{\boldsymbol{x}}}
\newcommand{\yx}{\ensuremath{y(\vecx)}}
\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace}           % domain / search space

% already defined in basic-math:
% \newcommand{\yv}{\boldsymbol{y}}
\newcommand{\fhx}{\ensuremath{\fh(\xv)}\xspace}            % surrogate (x), better use \mhx for predicted value



\newcommand{\minit}{m_{\text{init}}}											% Size of the initial design
\newcommand{\lambdai}{\lambdab^{[i]}}											% input for black box optimization 
\newcommand{\lambdanew}{\lambdab^{\text{new}}}								% new proposed configuration
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\lambdab^{[1]}, ..., \lambdab^{[\minit]}}  % Vector of different inputs
\newcommand{\lambdab}{\boldsymbol{\lambda}}									% input 
\newcommand{\lambdaopt}{\lambdab^{*}}											% Minimum of the black box function Psi


==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector

\newcommand{\biasc}{c}                          % bias in output


\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)

\newcommand{\Wmat}{\mathbf{W}}                             % weight vector (general)


\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Loss}{L(y, f(\xv, \thetab))}
\newcommand{\Lmomentumnest}{L(\yi, f(x^{(i)}, \thetab + \varphi \nub))}                  % momentum risk
\newcommand{\Lmomentumtilde}{L(\yi, f(x^{(i)}, \tilde{\thetab}))}                  % Nesterov momentum risk
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \thetab))} 
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\nub}{\boldsymbol{\nu}}

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function

% deeplearning - adversarials 
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\Lossdeltai}{L(\yi, f(\xi + \deltab|\thetab))}
\newcommand{\Lossdelta}{L(y, f(\xv + \deltab| \thetab))}

==> latex-math/ml-rf.tex <==
% ml -  ensemble methods, random forest

\newcommand{\betam}{\beta^{[m]}}												% baselearner with argument for m
\newcommand{\betaM}{\beta^{[M]}}												% baselearner with argument for M
\newcommand{\betai}{\beta^{[1]}}												% baselearner with argument for 1


==> latex-math/ml-survival.tex <==
\newcommand{\Ti}[1][i]{T^{(#1)}}
\newcommand{\Ci}[1][i]{C^{(#1)}}  
\newcommand{\oi}[1][i]{o^{(#1)}}  
\newcommand{\ti}[1][i]{t^{(#1)}}  
\newcommand{\lambdai}[1][i]{\lambda^{(#1)}}  
\newcommand{\deltai}[1][i]{\delta^{(#1)}}  
\newcommand{\Lxdi}{L\left(\bm{\delta}, \fx\right)}           



==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
% \newcommand{\HS}{\mathcal{H}}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Npk}{\Np_k}														% node N_k
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\pi_k^{(\Np)}}                                           		% class probability node N
\newcommand{\pikNh}[1][k]{\hat\pi_#1^{(\Np)}}                                           % estimated class probability node N
\newcommand{\pikNlh}[1][k]{\hat\pi_#1^{(\Nl)}}
\newcommand{\pikNrh}[1][k]{\hat\pi_#1^{(\Nr)}}

==> latex-math/probmodel.tex <==


% gaussians
\newcommand{\muk}{\bm{\mu_k}}  

